A note on the role of projectivity in likelihood-based inference for random graph models

There is widespread confusion about the role of projectivity in likelihood-based inference for random graph models. The confusion is rooted in claims that projectivity, a form of marginalizability, may be necessary for likelihood-based inference and consistency of maximum likelihood estimators. We show that likelihood-based superpopulation inference is not affected by lack of projectivity and that projectivity is not a necessary condition for consistency of maximum likelihood estimators.

==> preamble.tex <==
\usepackage{amsmath}
\usepackage{amssymb}
\RequirePackage[mathscr]{eucal}
\usepackage{csquotes}

%% Please use the following statements for
%% managing the text and math fonts for your papers:
\usepackage{times}
%\usepackage[cmbold]{mathtime}
\usepackage{bm}
\usepackage{natbib}


% General math operators
\def\grad{\bm{\nabla}}
\def\E{\mathbb{E}} % Expectation
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\logit}{logit}
\DeclareMathOperator{\N}{N} % Normal
\DeclareMathOperator{\Geometric}{Geometric}
\DeclareMathOperator{\Multinomial}{Multinomial}
\DeclareMathOperator{\Inv}{Inv}
\DeclareMathOperator{\MVN}{MVN}
\DeclareMathOperator{\Bernoulli}{Bernoulli}
\DeclareMathOperator{\Exponential}{Exponential}
\DeclareMathOperator{\ERGM}{ERGM}
\DeclareMathOperator{\RandomChoose}{RandomChoose}
\DeclareMathOperator{\0}{\mathbf{0}}
\DeclareMathOperator{\1}{\mathbf{1}}
\def\iid{{\stackrel{\tiny\mathrm{i.i.d.}}{\sim}}}
\def\ind{{\stackrel{\mathrm{ind.}}{\sim}}}
\DeclareMathOperator{\LN}{LN}
\DeclareMathOperator{\InvChiSq}{Inv\chi^2}
\DeclareMathOperator{\Dirichlet}{Dirichlet}
\DeclareMathOperator{\Poisson}{Poisson}
\DeclareMathOperator{\Binomial}{Binomial}
\DeclareMathOperator{\Uniform}{Uniform}
\DeclareMathOperator{\Conv}{Conv}
\DeclareMathOperator{\Prob}{Pr} % Note that \Pr undersets subscripts.
\DeclareMathOperator{\lik}{\mathscr{L}}
\DeclareMathOperator{\Image}{Im}
\DeclareMathOperator{\wrt}{d}
\def\llik{\ell}
\DeclareMathOperator{\Odds}{Odds}
\DeclareMathOperator*{\argmax}{arg\,max}
\def\argmin{\arg\min}
\def\ilogit{\logit^{-1}}
\def\reals{\mathbb{R}}
\def\naturals{\mathbb{N}}
\def\BB{\mathbb{B}}
\def\sumsamp{ \sum_{\sampind=1}^\sampsize }
\def\meansamp{\frac{1}{\sampsize}\sumsamp}
\def\s{\vspace{.15cm}}
\def\indep{\perp\!\!\!\perp}
\newcommand{\condind}[3]{#1 \indep #2 \,|\, #3}
\providecommand{\abs}[1]{\lvert#1\rvert}
\providecommand{\Abs}[1]{\left\lvert#1\right\rvert}
\def\half{\frac{1}{2}}
\def\t{^\top} % Transpose
\def\c{^{\mathsf{c}}} % Complement
\def\inv{^{-1}} % Inverse
\def\defeq{\stackrel{\text{def}}{=}}
\newcommand{\fromthru}[2]{\left\{#1\,..\,#2\right\}}
\newcommand{\innerprod}[2]{#1\t#2}
\newcommand{\powset}[1]{2^{#1}}

% Enclose the third argument into parentheses of the first and the
% second, scaling them for capital \EN.
% For example, \en(){1+1} -> "(1+1)", and \en[]{1+1} -> "[1+1]".
\newcommand{\EN}[3]{\left#1 #3 \right#2}
\newcommand{\en}[3]{#1 #3 #2}

\def\vertgroup{\mathscr{A}}
\def\verts{\mathscr{N}}
\def\attrf{\mathscr{X}}
\def\attrs{\bm{x}}
\def\Attrs{\bm{X}}
\def\nparf{ Q }
\def\npar{ q }
\def\edgeset{R}
\def\edgesetf{\bm{R}}
\def\param{\theta}
\def\paramf{\bm{\Theta}}
\def\params{\bm{\param}}
\def\genstat{s}
\def\genstats{\bm{\genstat}}
\def\genstatf{\mathbb{S}}
\def\netsetf{\mathbb{S}}
\def\dyadset{\mathcal{D}}
\def\netset{\mathcal{Y}}
\def\mreff{\mathbb{H}}
\def\mref{\nu}
\def\edgevals{\mathcal{S}}
\def\denspar{\pi}
\newcommand{\be}{\begin{equation}\begin{array}{lllllllllllllllll}}
\newcommand{\ee}{\end{array}\end{equation}}
\newcommand{\bX}{\bm{X}}
\newcommand{\bx}{\bm{x}}
\newcommand{\dprod}{\prod}
\newcommand{\dsum}{\sum}
\def\mR{\mathbb{R}}
\def\one{\mathbb{1}}

% ERGM ingredients
\newcommand{\edge}[1]{y_{#1}}
\newcommand{\Edge}[1]{Y_{#1}}
\def\net{y}
\def\Net{Y}
%% \def\netset{\mathcal{\Net}}
\def\attr{\bm{x}}
\def\weight{\bm{w}}
\def\esteq{\bm{U}}
% Asympotic notation
\def\subactors{ N }
\def\nactors{ n }
\def\actors{ \mathbb{N} }
\def\cnmapel{\eta}
\def\cnmap{\eta}
\def\dcnmap{\cnmap'}
\def\nnatpar{ p }
\def\curvparel{\theta}
\def\curvpar{{\bm{\curvparel}}}
\def\curvpars{\bm{\Theta}}
\def\natcurvpars{\bm{\Theta}_{\text{N}}}
\def\mle{\hat{\curvpar}}
\def\mple{\tilde{\curvpar}}
\def\designpar{\bm{\psi}}
\def\diffstat{z}
\def\diffstats{\bm{\diffstat}}
\def\target{\bm{t}}
\def\Design{\bm{D}}
\def\design{\bm{d}}
\def\maxdyadvals{ s }
\def\Borel{ \mathfrak{B} }
\def\changeij{\bm{\Delta}\sij\;}
\def\ipromotej{\bm{\Delta}\sij^\nearrow}
\def\normc{\kappa}
\def\lnormc{\psi}



% Measure-theoretic notation
\def\M{\mathbb{P}}
\def\nulldens{h}
\def\Mteg{\M_{\curvpar;\cnmap,\genstats}}
\def\Mtheg{\M_{\curvpar;\nulldens,\cnmap,\genstats}}
\def\Mref{\M_\nulldens}
\def\sigY{\mathsf{Y}}
\def\Mct{\tau}
\def\Mlbg{\lambda}
\def\drefdct{\frac{d\Mref}{d\Mct}}
\def\drefdlbg{\frac{d\Mref}{d\Mlbg}}
\def\dtegdref{\frac{d\Mteg}{d\Mref}}
\def\dtegdct{\frac{d\Mteg}{d\Mct}}

\newcommand{\natpar}[1][]{\cnmap#1(\curvpar)}
\newcommand{\natparT}[2][]{\cnmap#1(\curvpar^{#2})}
\newcommand{\natparp}[1][]{\cnmap#1(\curvpar')}
\newcommand{\natmle}[1][]{\cnmap#1(\mle)}
\newcommand{\dnatpar}[1][]{\dcnmap#1(\curvpar)}
\newcommand{\dnatparT}[2][]{\dcnmap#1(\curvpar^{#2})}
\newcommand{\dnatparp}[1][]{\dcnmap#1(\curvpar')}
\newcommand{\dnatmle}[1][]{\dcnmap#1(\mle)}


% Probabilities and expectations:
% P = probability, E = expectation, f = density, D = distribution, c = normalizing constant
\def\Pt{\Prob_{\curvpar}}
\def\Et{\E_{\curvpar}}
\def\ft{f_{\curvpar}}
\def\D{\ERGM}

\def\Pty{\Prob_{\curvpar;\netset}}
\def\Ety{\E_{\curvpar;\netset}}
\def\Vty{\Var_{\curvpar;\netset}}
\def\fty{f_{\curvpar;\netset}}
\def\Dy{\ERGM_{\netset}}
\def\cy{\normc_{\netset}}

\def\Py{\Prob_{\netset}}
\def\Ey{\E_{\netset}}
\def\Vy{\Var_{\netset}}
\def\fy{f_{\netset}}

\def\ceg{\normc_{\cnmap,\genstats}}
\def\Deg{\ERGM_{\cnmap,\genstats}}

\def\cheg{\normc_{\nulldens,\cnmap,\genstats}}
\def\Pheg{\Prob_{\nulldens,\cnmap,\genstats}}
\def\Eheg{\E_{\nulldens,\cnmap,\genstats}}
\def\Vheg{\Var_{\nulldens,\cnmap,\genstats}}
\def\fheg{f_{\nulldens,\cnmap,\genstats}}

\def\Dyheg{\ERGM_{\netset,\nulldens,\cnmap,\genstats}}
\def\cyheg{\normc_{\netset,\nulldens,\cnmap,\genstats}}
\def\Pyheg{\Prob_{\netset,\nulldens,\cnmap,\genstats}}
\def\Eyheg{\E_{\netset,\nulldens,\cnmap,\genstats}}
\def\Vyheg{\Var_{\netset,\nulldens,\cnmap,\genstats}}
\def\fyheg{f_{\netset,\nulldens,\cnmap,\genstats}}

% With optional arguments

\newcommand{\cY}[1]{\normc_{#1}}
\newcommand{\DY}[1]{\ERGM_{#1}}
\newcommand{\cYheg}[1]{\normc_{#1,\nulldens,\cnmap,\genstats}}
\newcommand{\DYheg}[1]{\ERGM_{#1,\nulldens,\cnmap,\genstats}}
\newcommand{\PY}[1]{\Prob_{#1}}
\newcommand{\EY}[1]{\E_{#1}}
\newcommand{\VY}[1]{\Var_{#1}}
\newcommand{\fY}[1]{f_{#1}}

% Subscripts, etc.

\def\ij{{i,j}}
\def\ji{{j,i}}
\def\pij{{(i,j)}}
\def\pji{{(j,i)}}
\def\ipjp{{i',j'}}
\def\pipjp{{(i',j')}}
\def\tij{\oplus\pij}
\def\ijedgespace{{\pij\in\edgespace}}
\def\netnetset{{\net\in\netset}}
\def\netpnetset{{\net'\in\netset}}
\def\sij{_{i,j}}
\def\sijk{_{i,j,k}}
\def\sik{_{i,k}}
\def\l{l}
\def\sil{_{i,\l}}
\def\sji{_{j,i}}
\def\sli{_{\l,i}}
\def\slj{_{\l,j}}
\def\slk{_{\l,k}}
\def\sipjp{_{i',j'}}
\def\Netij{Y\!\sij}
\def\netij{y\sij}
\def\Netji{Y\!\sji}
\def\netji{y\sji}
\def\nettij{\net\tij}
\def\Netnetij{\Netij=\netij}
\def\Nety{\Net=\net}


% Estimation
\def\sobs{^{\text{obs}}}
\def\smis{^{\text{mis}}}
\def\ssim{^{\text{sim}}}
\def\Netobs{\Net\sobs}
\def\netobs{\net\sobs}
\def\Netmis{\Net\smis}
\def\netmis{\net\smis}
\def\Netnetobs{\Netobs=\netobs}
\def\guessind{t}
\def\guess{\curvpar^\guessind}
\def\firstguess{\curvpar^0}
\def\firstguessel{\curvparel^0}
\def\nextguess{\curvpar^{\guessind+1}}
\def\netguess{\netseq^{\guess}}
\def\Netguess{\Netseq^{\guess}}
\def\meanee{\bar{\esteq}}
\def\mcmleee{\hat{\esteq}}
\def\pseudoee{\tilde{\esteq}}
\def\cdee{\esteq_{\shortmcmc{\cdpars}}}
\def\mcmlecdee{\hat{\esteq}_{\shortmcmc{\cdpars}}}
\def\mcmleE{\hat{\E}}

\def\mS{\mathscr{S}}
\def\mA{\mathscr{A}}
\def\mB{\mathscr{B}}
\def\mI{\mathscr{C}}
\def\mC{\mathscr{C}}
\def\mK{\mathscr{K}}
\def\mL{\mathscr{L}}
\def\mD{\mathscr{L}}
\def\mX{\mathcal{Y}}
\def\netspace{\mathcal{Y}}
\newcommand{\myexp}[1]{\exp\left(#1\right)}
\def\dint{\int}
\def\dfrac{\frac}
\newcommand{\I}[1]{1_{#1}}

\newcommand{\pkg}[1]{\texttt{#1}}
\newcommand{\proglang}[1]{\textsf{#1}}

% Coefficient table typesetting
\newcommand{\centercol}[1]{\multicolumn{1}{c}{#1}}
\newcommand{\coef}[2]{$#1$ $(#2)$}
\newcommand{\scoef}[2]{$\mathbf{#1}$ $(#2)$}

\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\eqs{\;=\;}
\def\neqs{\;\ne\;}
\def\proptos{\;\propto\;}
\def\bi{\begin{itemize}}
	\def\ei{\end{itemize}}
\def\mA{\mathscr{A}}
\def\mbE{\mathbb{E}}
\def\bmu{\bm\mu}
% Correctly typeset ``Erdos-Renyi''.
\def\ErRe{Erd\H{o}s--R\'{e}nyi}
\def\dis{\displaystyle}
\newcommand{\hide}[1]{}

\def\ndyadsn{\abs{\dyadset_{|\verts|}}} 
\def\ndyadsninv{\ndyadsn\inv\,} 
\def\ndyadsninvinv{\ndyadsn^{-2}\,} 
\newcommand{\ip}{\mathop{\to}\limits^{\mbox{\footnotesize p}}}
\def\mE{\dyadset}
\def\define{\mathop{=}\limits^{\mbox{\tiny def}}}
\def\Design{\bm{A}}
\def\design{\bm{a}}
\def\Designij{A_{i,j}}
\def\Designji{A_{j,i}}
\newcommand{\norm}[1]{\lVert#1\rVert}
\def\balpha{\bm{\alpha}}
\newcounter{com}
\newenvironment{com}[1][]{\refstepcounter{com}\par\medskip\indent%
	\textit{Remark~\thecom #1}. \rmfamily}{\medskip}

%\newcounter{theorem}
%\newenvironment{theorem}[1][]{\refstepcounter{theorem}\par\medskip\indent%
%\textbf{Theorem~\thetheorem #1}. \rmfamily}{\medskip}

%\newcounter{proposition}
%\newenvironment{proposition}[1][]{\refstepcounter{proposition}\par\medskip\indent%
%\textbf{Proposition~\theproposition #1}. \rmfamily}{\medskip}

\def\ooo{\net_{\verts'}}
\def\OOO{\Net_{\verts'}}

